An Empirical Study towards Characterizing Deep Learning Development and Deployment across Different Frameworks and Platforms

Deep Learning (DL) has recently achieved tremendous success. A variety of DL frameworks and platforms play a key role to catalyze such progress. However, the differences in architecture designs and implementations of existing frameworks and platforms bring new challenges for DL software development and deployment. Till now, there is no study on how various mainstream frameworks and platforms influence both DL software development and deployment in practice. To fill this gap, we take the first step towards understanding how the most widely-used DL frameworks and platforms support the DL software development and deployment. We conduct a systematic study on these frameworks and platforms by using two types of DNN architectures and three popular datasets. (1) For development process, we investigate the prediction accuracy under the same runtime training configuration or same model weights/biases. We also study the adversarial robustness of trained models by leveraging the existing adversarial attack techniques. The experimental results show that the computing differences across frameworks could result in an obvious prediction accuracy decline, which should draw the attention of DL developers. (2) For deployment process, we investigate the prediction accuracy and performance (refers to time cost and memory consumption) when the trained models are migrated/quantized from PC to real mobile devices and web browsers. The DL platform study unveils that the migration and quantization still suffer from compatibility and reliability issues. Meanwhile, we find several DL software bugs by using the results as a benchmark. We further validate the results through bug confirmation from stakeholders and industrial positive feedback to highlight the implications of our study. Through our study, we summarize practical guidelines, identify challenges and pinpoint new research directions.

==> tables-other.tex <==
	\begin{table}[t]
    \centering
		\scriptsize
		\setlength\tabcolsep{2.1pt}
		\caption{The hyper-parameters for DNN models on MNIST and CIFAR-10}
		\vspace{-2mm}
		\label{tbl:para1}
		\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
			\hline
			{\bf Dataset}&{\bf Mod.}  & {\bf Opt.} & {\bf Momt.} & {\bf LR.} & {\bf B.Sz.} & {\bf Epc.} & {\bf Drop.} & {\bf Wt.Dec.} & {\bf Tra.Para.}\\ \hline \hline
		    \multirow{2}{*}{\bf MNIST} &{\bf LeNet-1} & SGD & 9e-1 & 5e-2 & 128 & 200 & - & - & 3,246 \\ \cline{2-10}
		    &	{\bf LeNet-5} & SGD & 9e-1 & 5e-2 & 128 & 200 & - & - & 44,426\\ \hline
			\multirow{2}{*}{\bf CIFAR-10} & {\bf ResNet-20} & SGD & 9e-1 & 1e-1 & 128 & 200 & - & 1e-4 & 273,066 \\ \cline{2-10}
			&{\bf VGG-16} & SGD & 9e-1 & 1e-1 & 128 & 200 & 5e-1 & 1e-4 & 33,663,070  \\ \hline
		\end{tabular}
		\begin{tablenotes}
	\item Mod.: DNN models; Opt.: optimizer; Momt.: momentum; LR.: learning rate;  B.Sz: batch size; Epc.: epochs; Drop.: droupout; Wt.Dec.: weight decy; Tra.Para.: trainable parameters
\end{tablenotes}
	\vspace{-2mm}
	\end{table}
	
	
\begin{table}[t]
		\scriptsize
		\centering
		\setlength\tabcolsep{3.9pt}
		\caption{The hyper-parameters for DNN models on IMDb}
		\vspace{-2mm}
		\label{tbl:para2}
		\begin{tabular}{c|c|c|c|c|c|c|c|c}
			\hline
			{\bf Mod.} & {\bf Opt.} & {\bf LR.} & {\bf B.Sz.} & {\bf Epc.} & {\bf Drop.} & \textbf{Emb.Sz.} & \textbf{Stc.Len.} & {\bf Tra.Para.}\\ \hline \hline
		\textbf{TextCNN} & Adam  & 8e-5  & 256  & 30 & 5e-1 & 300 & 300 & 3,575,106 \\ \hline
			\textbf{GRU} & Adam  & 3e-4  & 256  & 30 & 5e-1 & 300 & 300 & 3,856,578 \\ \hline
			\textbf{LSTM} & Adam  & 8e-5  & 256  & 30 & 5e-1 & 300 & 300 & 4,141,762 \\ \hline
		\end{tabular}
		\begin{tablenotes}
		\item Mod.: DNN models; Opt.: optimizer; LR.: learning rate;  B.Sz: batch size; Epc.: epochs; Drop.: droupout; Emb.Sz.: embedding size; Stc.Len.: sentence length; Tra.Para.: trainable parameters
		\end{tablenotes}
% 		\vspace{-3mm}
\end{table}




\begin{table}
\centering
\tiny
\setlength\tabcolsep{4.0pt}
\caption{\small The output results of ResNet-20 on PC and Chrome}
\label{tbl:resnet20-diff}
\vspace{-2mm}
\begin{tabular}{c|c|c|c|c}
\hline
{\bf La.} & \multicolumn{2}{c|}{\textbf{Conv2D (First Weight Layer)}} & \multicolumn{2}{c}{\textbf{Dense (Last Weight Layer)}} \\ \hline
{\bf Pl.} & PC & Chrome & PC & Chrome \\ \hline \hline
 & 1.7837144136428833 & 1.7837144136428833 & 3.9491798877716064 & -1.0381317138671875 \\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -1.4785903692245483} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -1.478590488433838} & -5.77517032623291 & -3.2228665351867676 \\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.5716337561607361} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.5716336965560913} & 5.100228309631348 & \multicolumn{1}{>{\columncolor{mygray}}c}{\bf 3.760645627975464}\\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -0.013945930637419224} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -0.013945949263870716}  & -2.7495052814483643 & 1.5639196634292603 \\ \cline{2-5} 
 & -2.4287257194519043 & -2.4287257194519043 & 3.0477116107940674 & -1.4732520580291748 \\ \cline{2-5} 
 & ... & ... & -2.040926218032837 & 0.5265661478042603 \\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.003037585411220789} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.0030375919304788113} & -6.0745158195495605 & -0.17675308883190155 \\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -0.4366595149040222} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -0.4366595447063446} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 8.463834762573242} & 2.480924367904663 \\ \cline{2-5} 
 & 0.08801107853651047 & 0.08801107853651047 & -0.2396175116300583 & 1.3854891061782837 \\ \cline{2-5} 
\multirow{-10}{*}{\rotatebox{90}{\bf Layer Output}} &\multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.1746823787689209}  & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.1746823936700821} & -3.680608034133911 & -3.806004762649536 \\ \hline
\end{tabular}
\begin{tablenotes}
	\item La.: layer; Pl.: platform
\end{tablenotes}
%\vspace{-2mm}
\end{table}


\begin{table}
\centering
\scriptsize
\setlength\tabcolsep{7.2pt}
\caption{The layer outputs in ResNet-20 on \textsc{\small TensorFlow} model and \textsc{\small CNTK} variant}
\label{tbl:resnet20-diff-tf-cntk}
\vspace{-2mm}
\begin{tabular}{c|c|c|c|c}
\hline
{\bf Layer} & \multicolumn{2}{c|}{\textbf{Activation\_1}} & \multicolumn{2}{c}{\textbf{Dense (Last Weight Layer)}} \\ \hline
{\bf Framework} & \textbf{TensorFlow} & \textbf{CNTK} & \textbf{TensorFlow} & \textbf{CNTK} \\ \hline \hline
  & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 2.50329142} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 2.50329163} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 5.7574983} & 1.9206836 \\ \cline{2-5} 
 & 0.0 & 0.0 & 2.6037812 & -0.5768703 \\ \cline{2-5} 
 & 4.07436941 & 4.07436941 & -0.6758407 & 1.2657206 \\ \cline{2-5} 
 & 0.0 & 0.0 & 1.3866315 & 0.73824847 \\ \cline{2-5} 
 & 0.0 & 0.0 & -3.348287 & -0.97601014 \\ \cline{2-5} 
 & ... & ... & -4.9494123 & -3.5435727 \\ \cline{2-5} 
 & 0.0 & 0.0 & -2.8659112 & -1.4083405 \\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 3.72458271} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 3.72458232} & -4.317035 & -2.079543 \\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.62817883} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.62817895} & 4.1992025 & \multicolumn{1}{>{\columncolor{mygray}}c}{\bf 4.9673457} \\ \cline{2-5} 
\multirow{-10}{*}{\rotatebox{90}{\bf Layer Output}} & 1.00697954 & 1.00697954 & 2.2098625 & -0.3072039 \\ \hline
\end{tabular}
\end{table}






\begin{table}
\centering
\scriptsize
\setlength\tabcolsep{6.5pt}
\caption{\small The output results of ResNet-20 on PC and Chrome}
\label{tbl:resnet20-diff}
\vspace{-2mm}
\begin{tabular}{c|c|c|c|c}
\hline
{\bf Layer} & \multicolumn{2}{c|}{\textbf{Conv2D (First Weight Layer)}} & \multicolumn{2}{c}{\textbf{Dense (Last Weight Layer)}} \\ \hline
{\bf Platform} & PC & Chrome & PC & Chrome \\ \hline \hline
 & 1.78371441 & 1.78371441 & 3.94917989 & -1.03813171 \\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -1.47859037} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -1.47859049} & -5.77517033 & -3.22286654 \\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.57163376} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.57163370} & 5.10022831 & \multicolumn{1}{>{\columncolor{mygray}}c}{\bf 3.76064563}\\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -0.01394593} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -0.01394595}  & -2.74950528 & 1.56391966 \\ \cline{2-5} 
 & -2.42872572 & -2.42872572 & 3.04771161 & -1.47325206 \\ \cline{2-5} 
 & ... & ... & -2.04092622 & 0.52656615 \\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.003037585} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.003037592} & -6.07451582 & -0.17675309 \\ \cline{2-5} 
 & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -0.43665951} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf -0.43665954} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 8.46383476} & 2.48092437 \\ \cline{2-5} 
 & 0.08801108 & 0.08801108 & -0.23961751 & 1.38548911 \\ \cline{2-5} 
\multirow{-10}{*}{\rotatebox{90}{\bf Layer Output}} &\multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.174682378}  & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 0.174682394} & -3.68060803 & -3.80600476 \\ \hline
\end{tabular}
\end{table}


\begin{table}
\centering
\scriptsize
\setlength\tabcolsep{3.3pt}
\caption{Average of model size and training time}
\label{tbl:sizeandtime}
\begin{tabular}{c|c|c|c|c|c|c|c|c} 
\hline
\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}} \textbf{Models} \end{tabular}} & \multicolumn{2}{c|}{\textbf{TensorFlow} } & \multicolumn{2}{c|}{\textbf{CNTK} } & \multicolumn{2}{c|}{\textbf{PyTorch} } & \multicolumn{2}{c}{\textbf{MXNet}} \\ 
\cline{2-9}
 & \textbf{Size} & \textbf{Time}  & \textbf{Size} & \textbf{Time}  & \textbf{Size} & \textbf{Time}  & \textbf{Size} & \textbf{Time} \\ 
\hline\hline
 \textbf{LeNet-1}  & 16KB & 2.29 & 24KB & 2.26 & 24KB & 1.13 & 17KB & 0.98 \\ 
\hline
\textbf{LeNet-5}  & 178KB & 2.74 & 191KB & 2.64 & 186KB & 1.34 & 181KB & 1.07 \\ 
\hline
\textbf{ResNet-20}  & 1.1MB & 14.35 & 1.2MB & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 62.03} & 1.1MB & 11.77 & 1.1MB & \multicolumn{1}{>{\columncolor{mygray}}c}{\bf 9.81} \\ 
\hline
\textbf{VGG-16}  & 129MB & 26.17 & \multicolumn{1}{>{\columncolor{myother}}c|}{\bf 195MB} & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 249.69} & 129MB & 38.51 &  129MB & \multicolumn{1}{>{\columncolor{mygray}}c}{\bf 17.59} \\ 
\hline
\textbf{TextCNN}  & 14MB & 12.46 & 40MB & 13.64 & 13MB & 11.37 & \multicolumn{1}{>{\columncolor{myother}}c|}{\bf 1.9MB} & 10.82 \\ 
\hline
\textbf{LSTM}  & 16MB & 106.15 & 48MB & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 106.73} & 22MB & 53.02 & \multicolumn{1}{>{\columncolor{myother}}c|}{\bf 5.1MB} & \multicolumn{1}{>{\columncolor{mygray}}c}{\bf 25.78} \\ 
\hline
\textbf{GRU}  & 15MB & 231.27 & 29MB & \multicolumn{1}{>{\columncolor{mygray}}c|}{\bf 232.79} & 20MB & 45.90 & \multicolumn{1}{>{\columncolor{myother}}c|}{\bf 4.0MB} & \multicolumn{1}{>{\columncolor{mygray}}c}{\bf 24.06}  \\
\hline
\end{tabular}
%\begin{tablenotes}
	%\item Size: model size;  Time: training time (s) for each epoch
%\end{tablenotes}
\end{table}



